Towards Zero-shot Relation Extraction in Web Mining: A Multimodal Approach with Relative XML Path

The rapid growth of web pages and the increasing complexity of their structure poses a challenge for web mining models. Web mining models are required to understand the semi-structured web pages, particularly when little is known about the subject or template of a new page. Current methods migrate language models to the web mining by embedding the XML source code into the transformer or encoding the rendered layout with graph neural networks. However, these approaches do not take into account the relationships between text nodes within and across pages. In this paper, we propose a new approach, ReXMiner, for zero-shot relation extraction in web mining. ReXMiner encodes the shortest relative paths in the Document Object Model (DOM) tree which is a more accurate and efficient signal for key-value pair extraction within a web page. It also incorporates the popularity of each text node by counting the occurrence of the same text node across different web pages. We use the contrastive learning to address the issue of sparsity in relation extraction. Extensive experiments on public benchmarks show that our method, ReXMiner, outperforms the state-of-the-art baselines in the task of zero-shot relation extraction in web mining.

==> contents/deprecated-1-introduction.tex <==
% \section{Introduction}

% Internet carries rich information in different domains through semi-structured webpages where text nodes are distributed following HTML/XML markup language. Compared with plain text in the classic natural language understanding tasks, webpages are extended with multimodal features of the semi-structured visual and layout elements from HTML/XML source code, and these additional features can be well generalized between different websites.

% Due to the rapid updating pace of modern internet, it is unrealistic to annotate the emerging webpages and train a targeted web mining model for them. The web mining models are expected to deal with the open-domain information extraction task with little knowledge of the emerging subject or templates. Therefore, the multimodal features extracted from the HTML/XML source code along with the textual contents are the key to dealing with the open-domain task on the countless emerging webpages. 

% Previous approaches to this problem have focused on creating rich representations by modeling XML Paths of text nodes with large-scale pre-training. However, these methods fail to take into account the relative locality relationship within each webpage. Existing multimodal pre-training approaches extend the vanilla BERT with the embeddings of XML Path. The XML Path is a sequence of tags, e.g., \texttt{div}, \texttt{span}, \texttt{li}, indicating the location of the text node in the DOM Tree. In the relation extraction task, the related nodes are close to each other in the DOM Tree so their XML Paths have a long common prefix and the locality relationship is easy to be transfered to new webpages. Therefore, the relative XML Paths serve as a more efficient signal to prediction the relation between the text nodes. 

% Meanwhile, exiting web mining approaches ask the models to memorize various templates of webpages in the dataset but ignore the fact that webpages from the same website follow the same template. The relevance across different webpages of the same website can also be taken into consideration. We observe that a proportion of text nodes do not reveal any essential information about the subject but belong to the template so the specificity of each text should also be considered in the relation extraction task.

% To this end, we propose, OpenMiner, a new approach to tackle the open-domain relation extraction task from semi-structured webpages. We aim at learning the locality relationship within each webpage by exploiting the potential of DOM Tree of webpages. We extract the shortest path between text nodes as the relative XML Path, which removes the common prefix in the XML Paths of the text nodes and focuses on the relative relation. Following the relative position embedding in T5, we embed the relative XML Paths and the length of common prefix as attention bias in the multi-layered Transformer. We also incorporate the specificity of each text node by counting the number of times it occurs across different web pages. We embed the occurrence number logarithmically in the embedding layer, where we normalize the number and project it into a fixed number of embeddings. We also observe a serious data sparcity issue in the relation extraction task in web pages, where only a small proportion of text nodes are related to each other, and thus the number of negative cases is much larger than the positive one. To handle the data sparcity, we adopt the contrastive learning during training. We randomly generate the negative cases and restrict its ratio to the positive one. In this way, the model can properly discriminate the related text node pair against others.

% Learning from the relationships between text nodes within and across pages, our proposed model, OpenMiner, can properly transfer the knowledge learned from the existing websites to the new ones. We validate OpenMiner on websites about three different verticals from SWDE dataset, and the relation labels are annotated by CITE. We summarize our contribution as follows.

% \begin{itemize}[leftmargin=*,nosep]
%     \item We propose a novel multimodal framework that addresses the limitations of previous methods by effectively exploiting the relative locality relationship within each webpage and incorporating the specificity of text nodes in the relation extraction task.
%     % leverages the relative XML Paths from the DOM Tree and the occurrence number across different webpages to tackle the zero-shot relation extraction task in web mining.
%     \item We represent the relative locality relation and the specificity of text nodes in the language models through multimodal features from the relative XML Paths in the DOM Tree and the occurrence number of the text nodes across different web pages.
%     \item Extensive experiments on three different verticals from SWDE dataset demonstrate the effectiveness of OpenMiner in the zero-shot relation extraction task in web mining.
% \end{itemize}


==> tables/deprecated-tab-case_study2.tex <==
% Table generated by Excel2LaTeX from sheet 'case study'
\begin{table*}[htbp]
  \centering
    \small
\resizebox{\linewidth}{!}{
% Table generated by Excel2LaTeX from sheet 'Sheet5'
\begin{tabular}{lrllll}
\toprule
\multirow{2}[4]{*}{\textbf{Relative XML Path Pattern}} & \multirow{2}[4]{*}{} & \multicolumn{2}{c}{\textbf{w/ AbsXPath}} & \multicolumn{2}{c}{\textbf{w/ AbsXPath + RelXPath}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}      &       & \multicolumn{1}{c}{\textbf{Key}} & \multicolumn{1}{c}{\textbf{Value}} & \multicolumn{1}{c}{\textbf{Key}} & \multicolumn{1}{c}{\textbf{Value}} \\
\midrule
      &       & Color type & Technicolor prints & Color type & Technicolor prints \\
      &       & Moods	 & Food for Thought & Moods	 & Food for Thought \\
      &       &       &       & Genres & Drama \\
      & \multicolumn{1}{c}{\textit{True}}  &       &       & Flags & Adult Language \\
      & \multicolumn{1}{c}{\textit{Positive}} &       &       & Produced by & Buena Vista \\
      &       &       &       & Set In	 & 1958 \\
      &       &       &       & Sound by & Dolby \\
ABC   &       &       &       & Types & Americana \\
\cmidrule{2-6}
EFD   &       & Director & Drama & Director & Americana \\
      &       & Flags & Americana & Genres & Dolby \\
      & \multicolumn{1}{c}{\textit{False}} &       &       & MPAA Rating & Americana \\
      & \multicolumn{1}{c}{\textit{Negative}} &       &       & Moods	 & Technicolor prints \\
      &       &       &       & Tones & Technicolor prints \\
      &       &       &       & Types & Drama \\
\bottomrule
\end{tabular}%


% }
}
  \caption{Add caption}
  \label{tab:case}%
\end{table*}%


==> tables/tab-case_study.tex <==
% Table generated by Excel2LaTeX from sheet 'case study'
\begin{table*}[h]
  \centering
    \small
\resizebox{\linewidth}{!}{
    \setlength{\tabcolsep}{1mm}{
% Table generated by Excel2LaTeX from sheet 'Sheet6'
\begin{tabular}{rrcr}
\multicolumn{1}{l}{\textbf{\textit{NBA+Univ$\Rightarrow$Movie}}} &       &       &  \\
\midrule
\multicolumn{1}{l}{\textbf{Relative XML Path Pattern}} &       & \multicolumn{1}{l}{\textbf{ReXMiner w/ AbsXPath}} & \multicolumn{1}{l}{\textbf{ReXMiner w/ AbsXPath + RelXPath}} \\
\midrule
      & \multicolumn{1}{c}{\multirow{3}[2]{*}{\textit{True Positive}}} & \multicolumn{1}{l}{(color type, Technicolor prints); (Moods, } & \multicolumn{1}{l}{(color type, Technicolor prints); (Moods, Food for Thought)} \\
      &       & \multicolumn{1}{l}{Food for Thought)} & \multicolumn{1}{l}{(Genres, Drama); (Flags, Adult Language); (Produced by, } \\
\multicolumn{1}{l}{$\text{RelXPath}(x_i\Rightarrow x_j)$} &       &       & \multicolumn{1}{l}{Buena Vista); (Set In, 1958); (Sound by, Dolby)} \\
\cmidrule{2-4}\multicolumn{1}{l}{ = \texttt{[span;div;ul,li,a]}} & \multicolumn{1}{c}{\multirow{3}[2]{*}{\textit{False Positive}}} & \multicolumn{1}{l}{(Director, Drama); (Flags, Americana)} & \multicolumn{1}{l}{(Director, Americana); (Genres, Dolby); (MPAA Rating, } \\
      &       &       & \multicolumn{1}{l}{Americana); (Moods, Technicolor prints); (Types, Drama);} \\
      &       &       & \multicolumn{1}{l}{(Tones, Technicolor prints)} \\
\midrule
      &       & (a)   &  \\
\multicolumn{1}{l}{\textbf{\textit{Univ+Movie$\Rightarrow$NBA}}} &       &       &  \\
\midrule
\multicolumn{1}{l}{\textbf{Relative XML Path Pattern}} &       & \multicolumn{1}{l}{\textbf{ReXMiner w/ AbsXPath}} & \multicolumn{1}{l}{\textbf{ReXMiner w/ AbsXPath + RelXPath}} \\
\midrule
    & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textit{True Positive}}} & \multicolumn{1}{l}{\multirow{2}[2]{*}{(Wt:, 245)}} & \multicolumn{1}{l}{\multirow{2}[2]{*}{(Wt:, 245); (Ht:, 7' 0"); (Impact:, Barron agrain started ...)}} \\
\multicolumn{1}{l}{$\text{RelXPath}(x_i\Rightarrow x_j)$} &       &       &  \\
\cmidrule{2-4}\multicolumn{1}{l}{= \texttt{[;b;tail]}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textit{False Positive}}} & \multicolumn{1}{l}{\multirow{2}[2]{*}{(Bio, 245)}} & \multicolumn{1}{l}{\multirow{2}[2]{*}{(Ht:, 7' 0");}} \\
    &       &       &  \\
\midrule
    &       & (b)   &  \\
\end{tabular}%


}
}
  \caption{Add caption}
  \label{tab:case}%
\end{table*}%

